Controlling Chimeras

Coupled phase oscillators model a variety of dynamical phenomena in nature and technological applications. Non-local coupling gives rise to chimera states which are characterized by a distinct part of phase-synchronized oscillators while the remaining ones move incoherently. Here, we apply the idea of control to chimera states: using gradient dynamics to exploit drift of a chimera, it will attain any desired target position. Through control, chimera states become functionally relevant; for example, the controlled position of localized synchrony may encode information and perform computations. Since functional aspects are crucial in (neuro-)biology and technology, the localized synchronization of a chimera state becomes accessible to develop novel applications. Based on gradient dynamics, our control strategy applies to any suitable observable and can be generalized to arbitrary dimensions. Thus, the applicability of chimera control goes beyond chimera states in non-locally coupled systems.

==> arxiv accepted/commands.tex <==
% !TEX root = TravelingChimeraControl.tex
% CUSTOM COMMANDS AND THEOREMS (in separate file?)


% Theorems etc.

\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}

%\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{alg}[thm]{Algorithm}


%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{ex}[thm]{Example}

%\setlength{\theorempreskipamount}{10pt plus 1pt minus 1pt}
%\setlength{\theorempostskipamount}{8pt plus 1pt minus 1pt}
%\setlength{\bigskipamount}{10pt plus 2pt minus 2pt}
%\setlength{\medskipamount}{5pt plus 1pt minus 1pt}
%\setlength{\parskip}{10pt plus 1pt minus 1pt}
%\parindent 0 in

% Enumeration style (1), (2) etc.

%\renewcommand{\labelenumi}{(\arabic{enumi})}
%\renewcommand{\labelitemi}{$\diamond$}
%\newcommand{\fref}[1]{(F\ref{#1})}
\newcommand{\headerformat}[1]{\textsc{#1}}
%\renewcommand{\qedsymbol}{$\square$}
\newcommand{\thmheader}[1]{{#1}}
\newcommand{\lightthmheader}[1]{{\rm #1}}


\newcommand{\eqref}[1]{\eref{#1}}
\newcommand{\dotsc}{\ldots}
\newcommand{\text}{\textrm}

% MATHEMATICAL OPERATORS

\DeclareMathOperator{\mod}{mod}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\Rep}{Re}
\DeclareMathOperator{\Imp}{Im}
%\DeclareMathOperator{\tr}{trace}
%\DeclareMathOperator{\Jacc}{Jac}
\DeclareMathOperator{\Fix}{Fix}
\DeclareMathOperator{\Fx}{Fx}
\DeclareMathOperator{\coz}{coz}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Avg}{\Sigma}
\DeclareMathOperator{\FP}{Fix}
%\DeclareMathOperator{\FPx}{Fixm}
%\DeclareMathOperator{\EV}{Eigenvalues}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\RUB}{RUB}
%\DeclareMathOperator{\A}{A}
%\DeclareMathOperator{\B}{B}

\DeclareMathOperator*{\argmax}{arg\,max}

% SET SYMBOLS

\newcommand{\maxdim}{N}
%\newcommand{\maxdim}{\mathfrak{n}}

% Complex numbers and so on
\newcommand{\C}{\mathbb{C}}
\newcommand{\Cs}{\C^{\times}}
\newcommand{\Cn}{\C^\maxdim}
\newcommand{\Ch}{{\hat{\C}}}
\newcommand{\Cz}{\C[z]}
\newcommand{\Cm}{\C^{-}}
\newcommand{\Cme}{\C^{-e}}


\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zs}{\mathbb{Z}^{*}}
%\newcommand{\Zk}[1]{\Z_{#1}}
\newcommand{\Zk}[1]{\Z/{#1}\Z}
%\newcommand{\Zkdef}[1]{\Zk{#1} := \Z/#1\Z}
\newcommand{\Zkdef}[1]{\Zk{#1}}
\newcommand{\Zn}{\Zk{\maxdim}}

\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rr}{\R}
\newcommand{\Rn}{\R^\maxdim}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Hp}{\mathbb{H}}
\newcommand{\M}{\mathfrak{M}}
\newcommand{\Mdl}{\mathcal{M}}
\newcommand{\F}{\mathcal{F}}

% Tangent spaces
\newcommand{\Tg}{T}
\newcommand{\Tan}[1]{\Tg_{#1}}

% Torus
\newcommand{\Tor}{\mathbf{T}}
\newcommand{\Torn}{\Tor^{\maxdim}}
\newcommand{\Torno}{\Tor^{\maxdim-1}}
\newcommand{\Toro}{\Tor^{1}}

% Spheres
\renewcommand{\S}{\mathbf{S}}
\newcommand{\Sn}{\S^{\maxdim}}
\newcommand{\So}{\S^{1}}

% Permutation group
\newcommand{\Sym}[1]{S_{#1}}
\newcommand{\perm}{\mathfrak{p}}

% Misc
\newcommand{\B}{\mathbf{B}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Pts}{\Fx}


\newcommand{\OP}{Z}
\newcommand{\OPh}{{\OP}\ind{d}}
\newcommand{\aOP}{R}
\newcommand{\aOPh}{\aOP\ind{d}}
\newcommand{\I}{I}
\newcommand{\Ih}{\I\ind{d}}




% Abbreviations for convenience

\newcommand{\ud}{\mathrm{d}}
\newcommand{\si}[1]{\sigma_{i_{#1}}}
\newcommand{\s}{\sigma}
\newcommand{\ri}[2]{\varrho_{i_{#1}i_{#2}}}
\newcommand{\rh}{\varrho}
\renewcommand{\th}{\theta}
\newcommand{\rset}[2]{\left\lbrace\, #1\,\left|\;#2\right.\right\rbrace}
\newcommand{\lset}[2]{\left\lbrace\left. #1\;\right|\,#2\,\right\rbrace}
\newcommand{\set}[2]{\rset{#1}{#2}}
\newcommand{\tset}[2]{\big\lbrace #1\,\big|\;#2\big\rbrace}
\newcommand{\sset}[1]{\left\lbrace #1\right\rbrace}
\newcommand{\tsset}[1]{\big\lbrace #1\big\rbrace}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\tabs}[1]{\big| #1 \big|}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\ci}{\inv{c}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ph}{\varphi}
\newcommand{\G}{\Gamma}
\newcommand{\Rho}{P}
\newcommand{\io}{\iota}
\renewcommand{\Re}{\Rep}
\renewcommand{\Im}{\Imp}
\newcommand{\ind}[1]{_{\mathrm{#1}}}
\newcommand{\vphi}{\varphi}
\newcommand{\vrho}{\varrho}
\newcommand{\sr}{\vrho}
\newcommand{\srf}[2]{\sr_{#1}(#2)}
\renewcommand{\a}{{a}}
\newcommand{\xt}{x_*}

\newcommand{\lmax}{\lambda\ind{max}}
\newcommand{\lmaxh}{\hat{\lambda}\ind{max}}

\newcommand{\Jac}[1]{\ud #1}
\newcommand{\rev}{\vrho}
\newcommand{\Vt}{\widetilde{V}}
\newcommand{\Vws}{V^{\text{WS}}}
\newcommand{\PhiD}{\Phi}
\newcommand{\PsiD}{\Psi}
\renewcommand{\ph}{\Upsilon}



\DeclareMathOperator{\cso}{\mathbf{c}}
\DeclareMathOperator{\sno}{\mathbf{s}}
\DeclareMathOperator{\geo}{\mathbf{g}}
\newcommand{\cs}[2]{\cso_{#1}^{#2}}
\newcommand{\sn}[2]{\sno_{#1}^{#2}}
\newcommand{\sne}[1]{\sno_{#1}}
\newcommand{\SN}[1]{\mathcal{S}^{#1}}
\newcommand{\g}[1]{\geo_{#1}}


\newcommand{\dist}[2]{\left\|#1 - #2\right\|}
\newcommand{\FPm}[2]{\FPx_#1(#2)}
\newcommand{\sFP}{\FP^{\bullet}}
\renewcommand{\e}{\varepsilon}
\newcommand{\der}[1]{\frac{\ud}{\ud t}\left(#1\right)}
\newcommand{\ite}[2]{#1^{\circ #2}}
\newcommand{\xf}{{x^{*}}}
\newcommand{\yf}{{y^{*}}}
\newcommand{\zf}{{z^{*}}}
\newcommand{\alts}[1]{\hat{#1}}
\newcommand{\altw}[1]{\widehat{#1}}


\newcommand{\norm}[1]{\|#1\|}
\newcommand{\enorm}{\norm{\,\cdot\,}}
\newcommand{\esp}{\langle\,\cdot\,,\, \cdot\,\rangle}
\newcommand{\ball}[2]{B(#1, #2)}
\newcommand{\cball}[2]{\overline{\ball{#1}{#2}}}
\newcommand{\drv}[2]{\ud#1|_{#2}}

%\newcommand{\Fref}[1]{Figure~\ref{#1}}
%\newcommand{\Eref}[1]{Equation~\eqref{#1}}
%\newcommand{\eref}[1]{\eqref{#1}}
%\newcommand{\Sref}[1]{Section~\ref{#1}}

\newcommand{\pquad}{\qquad}


% Stalling parameters
\newcommand{\prn}{n}
\newcommand{\prm}{m}

\newcommand{\pn}[2]{#1 \backslash \!\left\lbrace #2\right\rbrace}
\newcommand{\FPs}{\FP^{*}}
%\newcommand{\imagescaling}{0.8}

\newcommand{\tf}{\tau_\textrm{fn}}
\newcommand{\Kf}{K_\textrm{fn}}
\newcommand{\OFx}{\OF_{\xf}}
\newcommand{\OFkt}{\OFx(K, \tau)}
\newcommand{\OFA}{\OF(x, K, \tau)}
\newcommand{\stb}{\chi}
\newcommand{\stba}{\hat\chi(x)}
\newcommand{\cj}[1]{{\overline{#1}}}

\newcommand{\OF}{\mathcal{Q}}
\newcommand{\Ob}{Q}
\newcommand{\Obf}{q}

\newcommand{\V}{\nu}
\newcommand{\Dt}{\Delta t}
\newcommand{\ah}{\hat{\a}}





